Automatic WSDL-guided Test Case Generation for PropEr Testing of Web Services

With web services already being key ingredients of modern web systems, automatic and easy-to-use but at the same time powerful and expressive testing frameworks for web services are increasingly important. Our work aims at fully automatic testing of web services: ideally the user only specifies properties that the web service is expected to satisfy, in the form of input-output relations, and the system handles all the rest. In this paper we present in detail the component which lies at the heart of this system: how the WSDL specification of a web service is used to automatically create test case generators that can be fed to PropEr, a property-based testing tool, to create structurally valid random test cases for its operations and check its responses. Although the process is fully automatic, our tool optionally allows the user to easily modify its output to either add semantic information to the generators or write properties that test for more involved functionality of the web services.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{J. Silva and and F. Tiezzi (Eds.): Workshop on Automated\\ 
Specification and Verification of Web Systems (WWV 2012)\\
EPTCS 98, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.98.3}{10.4204/EPTCS.98.3}}
\pdfoutput=1

